Surface Reconstruction from Point Clouds: A Survey and a Benchmark

Reconstruction of a continuous surface of two-dimensional manifold from its raw, discrete point cloud observation is a long-standing problem. The problem is technically ill-posed, and becomes more difficult considering that various sensing imperfections would appear in the point clouds obtained by practical depth scanning. In literature, a rich set of methods has been proposed, and reviews of existing methods are also provided. However, existing reviews are short of thorough investigations on a common benchmark. The present paper aims to review and benchmark existing methods in the new era of deep learning surface reconstruction. To this end, we contribute a large-scale benchmarking dataset consisting of both synthetic and real-scanned data; the benchmark includes object- and scene-level surfaces and takes into account various sensing imperfections that are commonly encountered in practical depth scanning. We conduct thorough empirical studies by comparing existing methods on the constructed benchmark, and pay special attention on robustness of existing methods against various scanning imperfections; we also study how different methods generalize in terms of reconstructing complex surface shapes. Our studies help identify the best conditions under which different methods work, and suggest some empirical findings. For example, while deep learning methods are increasingly popular, our systematic studies suggest that, surprisingly, a few classical methods perform even better in terms of both robustness and generalization; our studies also suggest that the practical challenges of misalignment of point sets from multi-view scanning, missing of surface points, and point outliers remain unsolved by all the existing surface reconstruction methods. We expect that the benchmark and our studies would be valuable both for practitioners and as a guidance for new innovations in future research.

==> figures/fig_exp_misalignment_wopre.tex <==
\begin{figure*}[hptb]
    \centering
    % \vspace{-0.3in}
    \begin{minipage}{0.94\linewidth}
        \centering
        \includegraphics[width=0.94\textwidth]{figures/figs/exp_fig_misalignment_wopre_part1.pdf}
        % \vspace{0.07in}
        \scalebox{0.67}{ \begin{tabular}{p{70pt}<{\centering}p{70pt}<{\centering}p{75pt}<{\centering}p{75pt}<{\centering}p{70pt}<{\centering}p{70pt}<{\centering}p{70pt}<{\centering}p{70pt}<{\centering}} \small Input PC & \    \small GT & \   \small GD \cite{greedydelaunay} & \     \small BPA \cite{BPA} &  \       \small SPSR \cite{kazhdan2013screened} &   \       \small RIMLS \cite{RIMLS}  &  \    \small SALD \cite{sald} &  \       \small IGR \cite{gropp2020implicitgeometricregularizationforlearningshape}    \\          \end{tabular}}
    \end{minipage}
    \vspace{-0.03in}

    \begin{minipage}{0.94\linewidth}
        \centering
        \includegraphics[width=0.94\textwidth]{figures/figs/exp_fig_misalignment_wopre_part2.pdf}
        % \vspace{0.07in}
        \scalebox{0.67}{\begin{tabular}{p{70pt}<{\centering}p{70pt}<{\centering}p{75pt}<{\centering}p{75pt}<{\raggedright}p{70pt}<{\centering}p{70pt}p{70pt}<{\centering}p{70pt}<{\centering}}  \small OccNet \cite{occupancy}  &  \       \small DeepSDF \cite{deepsdf}  &  \    \small LIG \cite{LIG} & \       \small Points2Surf \cite{points2surf} &  \         \small DSE \cite{learningdelaunaysurface} & \ \small IMLSNet \cite{liu2021DeepIMLS}  &  \       \small ParseNet \cite{parsenet} &  \       \small View Direction \\            \end{tabular}}
    \end{minipage}
    \vspace{-0.2cm}
    \caption{
        An example of qualitative results from different methods when dealing with the challenge of \textit{misalignment}.
        Note that the input point clouds are NOT pre-processed (cf. \cref{SecPreprocessing} for details).
    }
    \label{fig:misalig_wo_pre}
\end{figure*}


==> figures/fig_exp_missing_data_wopre.tex <==
\begin{figure*}[hptb]
    \centering
    % \vspace{-0.3in}
    \begin{minipage}{0.94\linewidth}
        \centering
        \includegraphics[width=0.94\textwidth]{figures/figs/exp_fig_missing_data_wopre_part1.pdf}
        % \vspace{0.07in}
        \scalebox{0.67}{ \begin{tabular}{p{70pt}<{\centering}p{70pt}<{\centering}p{75pt}<{\centering}p{75pt}<{\centering}p{70pt}<{\centering}p{70pt}<{\centering}p{70pt}<{\centering}p{70pt}<{\centering}} \small Input PC & \    \small GT & \   \small GD \cite{greedydelaunay} & \     \small BPA \cite{BPA} &  \       \small SPSR \cite{kazhdan2013screened} &   \       \small RIMLS \cite{RIMLS}  &  \    \small SALD \cite{sald} &  \       \small IGR \cite{gropp2020implicitgeometricregularizationforlearningshape}    \\          \end{tabular}}
    \end{minipage}
    \vspace{-0.03in}
    \begin{minipage}{0.94\linewidth}
        \centering
        \includegraphics[width=0.94\textwidth]{figures/figs/exp_fig_missing_data_wopre_part2.pdf}
        % \vspace{0.07in}
        \scalebox{0.67}{\begin{tabular}{p{70pt}<{\centering}p{70pt}<{\centering}p{75pt}<{\centering}p{75pt}<{\raggedright}p{70pt}<{\centering}p{70pt}p{70pt}<{\centering}p{70pt}<{\centering}}  \small OccNet \cite{occupancy}  &  \       \small DeepSDF \cite{deepsdf}  &  \    \small LIG \cite{LIG} & \       \small Points2Surf \cite{points2surf} &  \         \small DSE \cite{learningdelaunaysurface} & \ \small IMLSNet \cite{liu2021DeepIMLS}  &  \       \small ParseNet \cite{parsenet} &  \       \small GT \\            \end{tabular}}
    \end{minipage}
    \vspace{-0.2cm}
    \caption{
    An example of qualitative results from different methods when dealing with the challenge of \textit{missing points}.
    Note that the input point clouds are NOT pre-processed (cf. \cref{SecPreprocessing} for details).
    }
    \label{fig:missing_wo_pre}
\end{figure*}


==> figures/fig_exp_noise.tex <==
\begin{figure*}[htbp]
    \begin{minipage}{0.05\linewidth}
        \centering
        \scalebox{1.0}{\begin{tabular}{p{50pt}}
            \rotatebox{90}{\small learning-free} 
        \end{tabular}}
    \end{minipage}
    \begin{minipage}{0.01\linewidth}
        \centering
        \scalebox{0.8}{\begin{tabular}{p{2pt}}
            \rotatebox{90}{\small \ \ \ \ } \\[20pt]
            \rotatebox{90}{\small W/O defects} \\[65pt]
            \rotatebox{90}{\small Noise} \\[60pt]
        \end{tabular}}
    \end{minipage}
    \begin{minipage}{0.94\linewidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/figs/exp_fig_noise_part1.pdf}
        \vspace{0.07in}
        \scalebox{0.94}{ \begin{tabular}{p{70pt}<{\centering}p{70pt}<{\centering}p{75pt}<{\centering}p{75pt}<{\raggedright}p{70pt}<{\centering}p{70pt}<{\centering}}   \small GD \cite{greedydelaunay} & \     \small BPA \cite{BPA} &  \       \small SPSR \cite{kazhdan2013screened} &   \       \small RIMLS \cite{RIMLS} &    \  \small SALD \cite{sald} &  \       \small IGR \cite{gropp2020implicitgeometricregularizationforlearningshape}    \\          \end{tabular} }
    \end{minipage}
    \vspace{-0.02in}
    \begin{minipage}{0.05\linewidth}
        \centering
        \scalebox{1.0}{\begin{tabular}{p{50pt}}
            \rotatebox{90}{\small learning-based} 
        \end{tabular}}
    \end{minipage}
    \begin{minipage}{0.01\linewidth}
        \centering
        \scalebox{0.8}{\begin{tabular}{p{2pt}}
            \rotatebox{90}{\small \ \ \ \ } \\[20pt]
            \rotatebox{90}{\small W/O defects} \\[65pt]
            \rotatebox{90}{\small Noise} \\[60pt]
        \end{tabular}}
    \end{minipage}
    \begin{minipage}{0.94\linewidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/figs/exp_fig_noise_part2.pdf}
        \vspace{0.07in}
        \scalebox{0.94}{ \begin{tabular}{p{70pt}<{\centering}p{70pt}<{\centering}p{75pt}<{\centering}p{75pt}<{\raggedright}p{70pt}<{\centering}p{70pt}<{\centering}}   \small LIG \cite{LIG} & \       \small Points2Surf \cite{points2surf} &  \         \small DSE \cite{learningdelaunaysurface} & \ \small IMLSNet \cite{liu2021DeepIMLS} & \ \small Input PC & \   \small GT  \\            \end{tabular} }
    \end{minipage}
    \vspace{-0.01in}
    \caption{
    Qualitative results for synthetic datasets on clean data and imperfection of noisy. 
    The upper part of the figure shows the learning-free methods, and the lower part shows the learning-based methods; while for each method, we show the reconstruction results of clean data and imperfection of noise points.
    } 
    \label{fig:learning_based_vs_learning_free_noisy}
\end{figure*}


==> figures/fig_exp_noise_wopre.tex <==
\begin{figure*}[hptb]
    \centering
    % \vspace{-0.3in}
    \begin{minipage}{0.94\linewidth}
        \centering
        \includegraphics[width=0.94\textwidth]{figures/figs/exp_fig_noise_wopre_part1.pdf}
        % \vspace{0.07in}
        \scalebox{0.67}{ \begin{tabular}{p{70pt}<{\centering}p{70pt}<{\centering}p{75pt}<{\centering}p{75pt}<{\centering}p{70pt}<{\centering}p{70pt}<{\centering}p{70pt}<{\centering}p{70pt}<{\centering}} \small Input PC & \    \small GT & \   \small GD \cite{greedydelaunay} & \     \small BPA \cite{BPA} &  \       \small SPSR \cite{kazhdan2013screened} &   \       \small RIMLS \cite{RIMLS}  &  \    \small SALD \cite{sald} &  \       \small IGR \cite{gropp2020implicitgeometricregularizationforlearningshape}    \\          \end{tabular}}
    \end{minipage}
    \vspace{-0.03in}
    \begin{minipage}{0.94\linewidth}
        \centering
        \includegraphics[width=0.94\textwidth]{figures/figs/exp_fig_noise_wopre_part2.pdf}
        % \vspace{0.07in}
        \scalebox{0.67}{\begin{tabular}{p{70pt}<{\centering}p{70pt}<{\centering}p{75pt}<{\centering}p{75pt}<{\raggedright}p{70pt}<{\centering}p{70pt}p{70pt}<{\centering}p{70pt}<{\centering}}  \small OccNet \cite{occupancy}  &  \       \small DeepSDF \cite{deepsdf}  &  \    \small LIG \cite{LIG} & \       \small Points2Surf \cite{points2surf} &  \         \small DSE \cite{learningdelaunaysurface} & \ \small IMLSNet \cite{liu2021DeepIMLS}  &  \       \small ParseNet \cite{parsenet} &  \       \small GT \\            \end{tabular}}
    \end{minipage}
    \vspace{-0.2cm}
    \caption{
    An example of qualitative results from different methods when dealing with the challenge of \textit{point-wise noise}.
    Note that the input point clouds are NOT pre-processed (cf. \cref{SecPreprocessing} for details).
    }
    \label{fig:noise_wo_pre}
\end{figure*}


==> figures/fig_exp_outlier_wopre.tex <==
\begin{figure*}[hptb]
    \centering
    % \vspace{-0.3in}
    \begin{minipage}{0.94\textwidth}
        \centering
        \includegraphics[width=0.94\textwidth]{figures/figs/exp_fig_outlier_wopre_part1.pdf}
        % \vspace{0.07in}
        \scalebox{0.67}{ \begin{tabular}{p{70pt}<{\centering}p{70pt}<{\centering}p{75pt}<{\centering}p{75pt}<{\centering}p{70pt}<{\centering}p{70pt}<{\centering}p{70pt}<{\centering}p{70pt}<{\centering}} \small Input PC & \    \small GT & \   \small GD \cite{greedydelaunay} & \     \small BPA \cite{BPA} &  \       \small SPSR \cite{kazhdan2013screened} &   \       \small RIMLS \cite{RIMLS}  &  \    \small SALD \cite{sald} &  \       \small IGR \cite{gropp2020implicitgeometricregularizationforlearningshape}    \\          \end{tabular}}
    \end{minipage}
    \vspace{-0.03in}
    \begin{minipage}{0.94\textwidth}
        \centering
        \includegraphics[width=0.94\textwidth]{figures/figs/exp_fig_outlier_wopre_part2.pdf}
        % \vspace{0.07in}
        \scalebox{0.67}{\begin{tabular}{p{70pt}<{\centering}p{70pt}<{\centering}p{75pt}<{\centering}p{75pt}<{\raggedright}p{70pt}<{\centering}p{70pt}p{70pt}<{\centering}p{70pt}<{\centering}}  \small OccNet \cite{occupancy}  &  \       \small DeepSDF \cite{deepsdf}  &  \    \small LIG \cite{LIG} & \       \small Points2Surf \cite{points2surf} &  \         \small DSE \cite{learningdelaunaysurface} & \ \small IMLSNet \cite{liu2021DeepIMLS}  &  \       \small ParseNet \cite{parsenet} &  \       \small GT \\            \end{tabular}}
    \end{minipage}
    \vspace{-0.2cm}
    \caption{
        An example of qualitative results from different methods when dealing with the challenge of \textit{point outliers}.
        Note that the input point clouds are NOT pre-processed (cf. \cref{SecPreprocessing} for details).
    }
\label{fig:outliers_wo_pre}
\end{figure*}


==> figures/fig_exp_scene_wopre.tex <==
\begin{figure*}[htbp]
    \vspace{-0.2in}
    \begin{minipage}{0.05\linewidth}
        \centering
        \scalebox{0.7}{\begin{tabular}{p{50pt}}
            \rotatebox{90}{\small learning-free} \\[20pt]
        \end{tabular}}
    \end{minipage}
    \begin{minipage}{0.95\linewidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/figs/exp_fig_scene_wopre_part1.pdf}
        % \vspace{-0.05in}
        \scalebox{0.73}{ \begin{tabular}{p{70pt}<{\centering}p{70pt}<{\centering}p{75pt}<{\centering}p{75pt}<{\centering}p{70pt}<{\centering}p{70pt}<{\centering}p{70pt}<{\centering}p{70pt}<{\centering}} \small Input PC & \    \small GT & \   \small GD \cite{greedydelaunay} & \     \small BPA \cite{BPA} &  \       \small SPSR \cite{kazhdan2013screened} &   \       \small RIMLS \cite{RIMLS}  &  \    \small SALD \cite{sald} &  \       \small IGR \cite{gropp2020implicitgeometricregularizationforlearningshape}    \\          \end{tabular}}
        % \vspace{-0.02in}
    \end{minipage}
    % \vspace{-0.1in}
    \begin{minipage}{0.05\linewidth}
        \centering
        \scalebox{0.7}{\begin{tabular}{p{50pt}}
            \rotatebox{90}{\small learning-based} \\[20pt]
        \end{tabular}}
    \end{minipage}
    \begin{minipage}{0.95\linewidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/figs/exp_fig_scene_wopre_part2.pdf}
        \vspace{-0.05in}
        \scalebox{0.73}{\begin{tabular}{p{70pt}<{\centering}p{70pt}<{\centering}p{75pt}<{\centering}p{75pt}<{\raggedright}p{70pt}<{\centering}p{70pt}p{70pt}<{\centering}p{70pt}<{\centering}}  \small OccNet \cite{occupancy}  &  \       \small DeepSDF \cite{deepsdf}  &  \    \small LIG \cite{LIG} & \       \small Points2Surf \cite{points2surf} &  \         \small DSE \cite{learningdelaunaysurface} & \ \small IMLSNet \cite{liu2021DeepIMLS}  &  \       \small ParseNet \cite{parsenet} &  \       \small GT \\            \end{tabular}}
        % \vspace{-0.02in}
    \end{minipage}
    \vspace{-0.08in}
    \caption{
        Qualitative results respectively from optimization-based, learning-free methods and learning-based, data-driven methods on the testing synthetic data of scene surfaces that the input point clouds are NOT pre-processed (cf. \cref{SecPreprocessing} for details). The scene is a dining room instance from the 3D-FRONT \cite{3dfrontdata}.}
    \label{fig:opt_vs_learn_sce_wo_pre}
\end{figure*}


==> figures/fig_exp_wnoise_semantic_nonseman_wopre.tex <==
\begin{figure*}[htbp]
    \vspace{-0.2in}
    \begin{minipage}{0.05\linewidth}
        \centering
        \scalebox{1.0}{\begin{tabular}{p{50pt}}
            \rotatebox{90}{\small learning-free} \\[45pt]
        \end{tabular}}
    \end{minipage}\begin{minipage}{0.94\linewidth}
        \centering
        \includegraphics[width=0.98\textwidth]{figures/figs/exp_fig_wnoise_semantic_nonsematic_wopre_part1.pdf}
        \scalebox{0.70}{ \begin{tabular}{p{70pt}<{\centering}p{70pt}<{\centering}p{75pt}<{\centering}p{75pt}<{\centering}p{70pt}<{\centering}p{70pt}<{\centering}p{70pt}<{\centering}p{70pt}<{\centering}} \small Input PC & \    \small GT & \   \small GD \cite{greedydelaunay} & \     \small BPA \cite{BPA} &  \       \small SPSR \cite{kazhdan2013screened} &   \       \small RIMLS \cite{RIMLS}  &  \    \small SALD \cite{sald} &  \       \small IGR \cite{gropp2020implicitgeometricregularizationforlearningshape}    \\          \end{tabular}}
        % \vspace{-0.05in}
    \end{minipage}
    % \vspace{-0.05in}
    \begin{minipage}{0.05\linewidth}
        \centering
        \scalebox{1.0}{\begin{tabular}{p{50pt}}
            \rotatebox{90}{\small learning-based} \\[45pt]
        \end{tabular}}
    \end{minipage}
    \begin{minipage}{0.94\linewidth}
        \centering
        \includegraphics[width=0.98\textwidth]{figures/figs/exp_fig_wnoise_semantic_nonsematic_wopre_part2.pdf}
        \vspace{-0.05in}
        \scalebox{0.70}{\begin{tabular}{p{70pt}<{\centering}p{70pt}<{\centering}p{75pt}<{\centering}p{75pt}<{\raggedright}p{70pt}<{\centering}p{70pt}p{70pt}<{\centering}p{70pt}<{\centering}}  \small OccNet \cite{occupancy}  &  \       \small DeepSDF \cite{deepsdf}  &  \    \small LIG \cite{LIG} & \       \small Points2Surf \cite{points2surf} &  \         \small DSE \cite{learningdelaunaysurface} & \ \small IMLSNet \cite{liu2021DeepIMLS}  &  \       \small ParseNet \cite{parsenet} &  \       \small GT \\            \end{tabular}}
    \end{minipage}
    \vspace{-0.08in}
    \caption{
        Qualitative results respectively from optimization-based, learning-free methods and learning-based, data-driven methods on the testing synthetic data of object surfaces that the input point clouds are NOT pre-processed (cf. \cref{SecPreprocessing} for details). The input point clouds have imperfect scanning of \emph{point-wise noise}. The example of \emph{chair} is of popular semantic categories, for which our auxiliary training set contains rich instances of the same category from ShapeNet \cite{shapenet}; the other one is non-semantic.
    } 
    \label{fig:opt_vs_learn_obj_wo_pre}
\end{figure*}


==> figures/fig_result_midlevel_wopre.tex <==
\begin{figure}[hptb]
    % \vspace{-0.2in}
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/figs/fig_metrics_midlevel_wopre_CD.png}
        \subcaption{CD}
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/figs/fig_metrics_midlevel_wopre_F-score.png}
        \subcaption{F-score}
    \end{minipage}\\
    \vspace{-0.05in}
    \begin{minipage}{0.49\linewidth}
        \includegraphics[width=0.99\textwidth]{figures/figs/fig_metrics_midlevel_wopre_NCS.png}
        \subcaption{NCS}
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
        \includegraphics[width=0.99\textwidth]{figures/figs/fig_metrics_midlevel_wopre_NFS.png}
        \subcaption{NFS}
    \end{minipage}
    \vspace{-0.2cm}
    \caption{
        Plotting of quantitative results in \cref{tab:syn_obj_wo_preprocess} under different evaluation metrics. For those challenges with varying levels of severity, we use the data of middle-level severity for the comparison.
    }
    \label{fig:diff_metric_wo_pre}
\end{figure}


==> tables/tab_Noise_wopre.tex <==
\begin{table*}[hptb]
\centering
\caption{
Comparison between optimization-based, learning-free methods and learning-based, data-driven methods on the testing synthetic data of object surfaces that the input point clouds are Not preprocessed (cf. \cref{SecPreprocessing} for details). 
We report quantitative results for the imperfect scanning of \emph{point-wise noise} at three levels of severity; results are in the format of ``$\cdot$ / $\cdot$ / $\cdot$'', where the most left one is the absolute value under each evaluation metric, and the right two ones are those relative to the most left one. 
The \textbf{best} and \uline{\textbf{second best}} methods are highlighted in each column. 
}
\vspace{-0.1in}
\label{tab:noise_wopre}
\resizebox{0.94\textwidth}{!}{
\begin{tabular}{l|c|r@{ /}r@{ / }c|r@{ /}r@{ / }c|r@{ /}r@{ / }c|r@{ /}r@{ / }c}
\hline
\multirow{2}{*}{\makecell{Algorithms}} & \multirow{2}{*}{\makecell{Priors}} & \multicolumn{3}{c|}{CD $ (\times10^{-4}) \downarrow$} & \multicolumn{3}{c|}{F-score $(\%) \uparrow$} & \multicolumn{3}{c|}{NCS $ (\times10^{-2}) \uparrow$} & \multicolumn{3}{c}{NFS $ (\times10^{-2}) \uparrow$} \\\cline{3-14}
~ & ~ & \emph{\makecell{low-}} & \emph{\makecell{middle-}}  & \emph{\makecell{high-\\level}} &\emph{\makecell{low-}} & \emph{\makecell{middle-}} & \emph{\makecell{high-\\level}} & \emph{\makecell{low-}} & \emph{\makecell{middle-}} & \emph{\makecell{high-\\level}} & \emph{\makecell{low-}} & \emph{\makecell{middle-}} & \emph{\makecell{high-\\level}} \\\hline
GD \cite{greedydelaunay}                                               &   \multirow{6}{*}{\makecell{learning-\\free}}         & 21.39                        & 13.14                       & 25.27                       & 97.85                        & -11.32                       & -36.19                       & 80.31                        & -10.99                      & -22.98                       & 78.07                        & -28.09                      & -37.12                   \\ 
BPA \cite{BPA}                                                         &                                                       & 23.76                        & 25.66                       & 31.87                       & 92.90                        & -11.11                       & -30.85                       & 82.88                        & -9.74                       & -22.48                       & 77.09                        & -21.02                      & -33.31                   \\ 
SPSR \cite{kazhdan2013screened}                                        &                                                       & \textbf{15.89}               & 2.68                        & 7.10                        & \textbf{99.54}               & -0.18                        & -2.28                        & \uline{\textbf{95.89}}       & -2.38                       & -4.83                        & \textbf{94.84}               & -4.15                       & -9.31                    \\               
RIMLS \cite{RIMLS}                                                     &                                                       & 18.44                        & 7.94                        & 25.37                       & \uline{\textbf{98.88}}       & -4.08                        & -32.70                       & 93.10                        & -11.07                      & -23.09                       & 91.92                        & -16.77                      & -35.85                   \\ 
SALD \cite{sald}                                                       &                                                       & 22.98                        & 6.78                        & 20.18                       & 98.47                        & -9.67                        & -35.82                       & 90.35                        & -2.60                       & -12.78                       & 72.18                        & -7.17                       & -18.57                   \\                                 
IGR \cite{gropp2020implicitgeometricregularizationforlearningshape}    &                                                       & \uline{\textbf{18.29}}       & 1.62                        & 3.54                        & 98.26                        & -1.01                        & \uline{\textbf{-1.73}}       & \textbf{97.13}               & -0.14                       & -0.79                        & \uline{\textbf{94.13}}       & -0.17                       & -2.53                    \\ \hline  
OccNet \cite{occupancy}                                                &   \multirow{7}{*}{\makecell{learning-\\based}}        & 201.56                       & 12.62                       & 4.34                        & 30.37                        & -2.66                        & -5.36                        & 79.74                        & -0.42                       & \uline{\textbf{-0.15}}       & 47.29                        & -1.98                       & \uline{\textbf{-2.45}}   \\
DeepSDF \cite{deepsdf}                                                 &                                                       & 241.98                       & 2.27                        & 15.44                       & 16.37                        & -1.14                        & -4.02                        & 78.37                        & 0.00                        & -0.35                        & 38.20                        & -0.91                       & -2.86                    \\
LIG \cite{LIG}                                                         &                                                       & 26.99                        & 3.15                        & \uline{\textbf{2.72}}       & 92.37                        & -0.19                        & -3.64                        & 94.67                        & -0.42                       & -1.08                        & 89.19                        & -2.04                       & -3.14                    \\
Points2Surf \cite{points2surf}                                         &                                                       & 23.47                        & 1.74                        & 5.87                        & 93.94                        & \uline{\textbf{-0.17}}       & -2.77                        & 93.11                        & -0.27                       & -1.57                        & 90.28                        & -1.99                       & -3.93                    \\               
DSE \cite{learningdelaunaysurface}                                     &                                                       & 19.32                        & 8.22                        & 21.27                       & 98.87                        & -6.59                        & -30.03                       & 80.51                        & -10.86                      & -26.17                       & 81.08                        & -26.25                      & -40.64                   \\                                                                    
IMLSNet \cite{liu2021DeepIMLS}                                         &                                                       & 22.93                        & \uline{\textbf{1.06}}       & 10.16                       & 95.30                        & -0.86                        & -9.92                        & 95.20                        & \uline{\textbf{0.14}}       & -1.63                        & 90.08                        & \uline{\textbf{0.09}}       & -10.39                   \\
ParseNet \cite{parsenet}                                               &                                                       & 165.10                       & \textbf{-6.58}              & \textbf{-7.14}              & 41.24                        & \textbf{2.10}                & \textbf{-1.10}               & 78.33                        & \textbf{1.20}               & \textbf{1.09}                & 40.71                        & \textbf{6.02}               & \textbf{4.67}            \\\hline                                        
\end{tabular}%
}
\end{table*}                               




==> tables/tab_without_or_need_normal_scene_wopre.tex <==
\begin{table}[hptb]
\centering
\caption{
    Comparison between methods without using surface normals ($\times$), methods rely on surfaces normals ($\checkmark$), and methods only rely on surface normals during learning ($*$) on the testing synthetic data of scene surfaces that the input point clouds are Not preprocessed (cf. \cref{SecPreprocessing} for details).
    % We report quantitative results for the imperfect scanning of \emph{point-wise noise} at the middle-level of severity; 
    results are in the format of ``$\cdot$ / $\cdot$'', where the left one is obtained assuming the ground-truth camera poses, and the right one is obtained without knowing the relative camera poses. 
    The \textbf{best} and \uline{\textbf{second best}} methods are highlighted in each column. 
}
\vspace{-0.1in}
\label{tab:normal_sce_wo_pre}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c|c|c} \hline
\multirow{1}{*}{Algorithms} & \multirow{1}{*}{Normals} & \multicolumn{1}{c|}{CD $(\times10^{-3}) \downarrow$} & \multicolumn{1}{c|}{F-score $(\%) \uparrow$} & \multicolumn{1}{c|}{NCS $(\times10^{-2}) \uparrow$} & \multicolumn{1}{c}{NFS $(\times10^{-2}) \uparrow$} \\\hline
% ~ & ~ & \makecell{Point-wise\\noise} & \makecell{Point-wise\\noise} & \makecell{Perfect\\scanning} & \makecell{Non-uniform\\scanning} & \makecell{Point-wise\\noise}& \makecell{Perfect\\scanning} & \makecell{Non-uniform\\scanning} & \makecell{Point-wise\\noise}\\ \hline
GD \cite{greedydelaunay}                                                &  \multirow{3}{*}{$\times$}      & 34.50                       / {\ \ \ \ \ \ \ } & 71.33                     / {\ \ \ \ \ \ \ } & 56.78                     / {\ \ \ \ \ \ \ } & 38.77                    / {\ \ \ \ \ \ \ }    \\ 
SALD \cite{sald}                                                        &                                 & 32.87                       / {\ \ \ \ \ \ \ } & 75.15                     / {\ \ \ \ \ \ \ } & \textbf{91.29}            / {\ \ \ \ \ \ \ } & 51.36                    / {\ \ \ \ \ \ \ }    \\ 
DSE \cite{learningdelaunaysurface}                                      &                                 & 33.46                       / {\ \ \ \ \ \ \ } & 72.35                     / {\ \ \ \ \ \ \ } & 52.70                     / {\ \ \ \ \ \ \ } & 38.37                    / {\ \ \ \ \ \ \ }    \\ \hline
BPA \cite{BPA}                                                          &  \multirow{7}{*}{$\checkmark$}  & 49.01                       / 61.52            & 55.45                     / 48.85            & 53.52                     / 40.00            & 39.87                    / 28.57               \\ 
SPSR \cite{kazhdan2013screened}                                         &                                 & {\ }\textbf{30.63}          / 143.68           & \textbf{83.03}            / 67.83            & 83.50                     / 60.87            & \uline{\textbf{62.46}}   / 40.90               \\ 
RIMLS \cite{RIMLS}                                                      &                                 & 42.53                       / 57.46            & 69.74                     / 60.79            & 64.83                     / 47.88            & 33.82                    / 23.41               \\ 
IGR \cite{gropp2020implicitgeometricregularizationforlearningshape}     &                                 & {\ }\uline{\textbf{32.82}}  / 368.09           & \uline{\textbf{81.37}}    / 63.06            & \uline{\textbf{90.32}}    / 66.56            & \textbf{66.71}           / 41.63               \\
OccNet \cite{occupancy}                                                 &                                 & 102.75                      / 133.55           & 34.60                     / 29.51            & 85.01                     / 63.01            & 45.95                    / 33.20               \\
DeepSDF \cite{deepsdf}                                                  &                                 &  -                          / -                &       -                   / -                &       -                   / -                &        -                 / -                   \\ 
LIG \cite{LIG}                                                          &                                 & 42.03                       / 82.62            & 67.42                     / 54.98            & 74.84                     / 54.59            & 51.86                    / 34.19               \\ 
ParseNet \cite{parsenet}                                                &                                 &  -                          / -                &       -                   / -                &       -                   / -                &        -                 / -                   \\ \hline
Points2Surf \cite{points2surf}                                          &  \multirow{2}{*}{$*$}           & 39.60                       / {\ \ \ \ \ \ \ } & 75.00                     / {\ \ \ \ \ \ \ }  & 82.25                    / {\ \ \ \ \ \ \ } & 59.33                    / {\ \ \ \ \ \ \ }    \\ 
IMLSNet \cite{liu2021DeepIMLS}                                          &                                 & 36.22                       / {\ \ \ \ \ \ \ } & 75.04                     / {\ \ \ \ \ \ \ }  & 86.45                    / {\ \ \ \ \ \ \ } & 59.40                    / {\ \ \ \ \ \ \ }    \\ \hline
\end{tabular}%
}
\end{table}



==> tables/tab_without_or_need_normal_wopre.tex <==
\begin{table}[hptb]
\centering
\caption{
    Comparison between methods without using surface normals ($\times$), methods rely on surfaces normals ($\checkmark$), and methods only rely on surface normals during learning ($*$) on the testing synthetic data of object surfaces that the input point clouds are Not preprocessed (cf. \cref{SecPreprocessing} for details).
    We report quantitative results for the imperfect scanning of \emph{point-wise noise} at the middle-level of severity; 
    results are in the format of ``$\cdot$ / $\cdot$'', where the left one is obtained assuming the ground-truth camera poses, and the right one is obtained without knowing the relative camera poses. 
    The \textbf{best} and \uline{\textbf{second best}} methods are highlighted in each column. 
}
\vspace{-0.1in}
\label{tab:normal_obj_wo_pre}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c|c|c} \hline
\multirow{1}{*}{Algorithms} & \multirow{1}{*}{Normals} & \multicolumn{1}{c|}{CD $(\times10^{-4}) \downarrow$} & \multicolumn{1}{c|}{F-score $(\%) \uparrow$} & \multicolumn{1}{c|}{NCS $(\times10^{-2}) \uparrow$} & \multicolumn{1}{c}{NFS $(\times10^{-2}) \uparrow$} \\\hline
% ~ & ~ & \makecell{Point-wise\\noise} & \makecell{Point-wise\\noise} & \makecell{Perfect\\scanning} & \makecell{Non-uniform\\scanning} & \makecell{Point-wise\\noise}& \makecell{Perfect\\scanning} & \makecell{Non-uniform\\scanning} & \makecell{Point-wise\\noise}\\ \hline
GD \cite{greedydelaunay}                                                &  \multirow{3}{*}{$\times$}      & 34.53                        / {\ \ \ \ \ \ \ } & 86.53                        / {\ \ \ \ \ \ \ } & 69.32                     / {\ \ \ \ \ \ \ } & 49.98                       / {\ \ \ \ \ \ \ }        \\ 
SALD \cite{sald}                                                        &                                 & 29.76                        / {\ \ \ \ \ \ \ } & 88.80                        / {\ \ \ \ \ \ \ } & 87.75                     / {\ \ \ \ \ \ \ } & 65.01                       / {\ \ \ \ \ \ \ }        \\ 
DSE \cite{learningdelaunaysurface}                                      &                                 & 27.54                        / {\ \ \ \ \ \ \ } & 92.28                        / {\ \ \ \ \ \ \ } & 69.65                     / {\ \ \ \ \ \ \ } & 54.83                       / {\ \ \ \ \ \ \ }        \\ \hline
BPA \cite{BPA}                                                          &  \multirow{7}{*}{$\checkmark$}  & 49.42                        / 49.89            & 81.79                        / 81.65            & 73.14                     / 73.19            & 56.07                       / 54.04                   \\ 
SPSR \cite{kazhdan2013screened}                                         &                                 & \textbf{18.57}               / 70.16            & \textbf{99.36}               / 90.88            & 93.51                     / 90.85            & \uline{\textbf{90.69}}      / 80.51                   \\ 
RIMLS \cite{RIMLS}                                                      &                                 & 26.38                        / 28.94            & 94.80                        / 92.80            & 82.03                     / 80.92            & 75.15                       / 70.02                   \\ 
IGR \cite{gropp2020implicitgeometricregularizationforlearningshape}     &                                 & {\ } \uline{\textbf{19.91}}  / 281.35           & \uline{\textbf{97.25}}       / 85.37            & \textbf{96.99}            / 94.65            & \textbf{93.96}              / 78.77                   \\
OccNet \cite{occupancy}                                                 &                                 & 214.18                       / 223.85           & 27.71                        / 26.78            & 79.32                     / 78.38            & 45.31                       / 44.35                   \\
DeepSDF \cite{deepsdf}                                                  &                                 & 244.25                       / 604.06           & 15.23                        / 13.47            & 78.37                     / 77.45            & 37.29                       / 32.06                   \\ 
LIG \cite{LIG}                                                          &                                 & 30.14                        / 47.62            & 92.18                        / 85.01            & 94.25                     / 91.35            & 87.15                       / 77.59                   \\ 
ParseNet \cite{parsenet}                                                &                                 & 158.52                       / 230.29           & 43.34                        / 35.02            & 79.53                     / 75.28            & 46.73                       / 39.11                   \\ \hline
Points2Surf \cite{points2surf}                                          &  \multirow{2}{*}{$*$}           & 25.21                        / {\ \ \ \ \ \ \ } & 93.77                        / {\ \ \ \ \ \ \ } & 92.84                     / {\ \ \ \ \ \ \ } & 88.29                       / {\ \ \ \ \ \ \ }        \\ 
IMLSNet \cite{liu2021DeepIMLS}                                          &                                 & 23.99                        / {\ \ \ \ \ \ \ } & 94.44                        / {\ \ \ \ \ \ \ } & \uline{\textbf{95.34}}    / {\ \ \ \ \ \ \ } & 90.17                       / {\ \ \ \ \ \ \ }        \\ \hline
\end{tabular}%
}
\end{table}

